VeriDL: Integrity Verification of Outsourced Deep Learning Services (Extended Version)

Deep neural networks (DNNs) are prominent due to their superior performance in many fields. The deep-learning-as-a-service (DLaaS) paradigm enables individuals and organizations (clients) to outsource their DNN learning tasks to the cloud-based platforms. However, the DLaaS server may return incorrect DNN models due to various reasons (e.g., Byzantine failures). This raises the serious concern of how to verify if the DNN models trained by potentially untrusted DLaaS servers are indeed correct. To address this concern, in this paper, we design VeriDL, a framework that supports efficient correctness verification of DNN models in the DLaaS paradigm. The key idea of VeriDL is the design of a small-size cryptographic proof of the training process of the DNN model, which is associated with the model and returned to the client. Through the proof, VeriDL can verify the correctness of the DNN model returned by the DLaaS server with a deterministic guarantee and cheap overhead. Our experiments on four real-world datasets demonstrate the efficiency and effectiveness of VeriDL.

==> practicalattack.tex <==
\section{Use Cases of Attacks}
\label{sc:practicalattack}
%So far we have shown that \system to detect Byzantine failures in the training process of federated learning. A good property of \system is that it is generic and is able to detect a wide range of attacks against DNN models. 
In this section, we discuss how \system can catch the incorrect model updates by three different types of attacks. 

\nop{
\noindent{\bf DNN backdoor attacks.}
Existing work \cite{bagdasaryan2018backdoor,liu2017trojaning,chen2017targeted,gu2017badnets} propose various methods to introduce stealthy backdoor functionality into a DNN model. The compromised model preserves the state-of-the-art performance on the normal user's validation data. However, at the presence of a backdoor input, the model's accuracy degrades significantly: it either produces an attacker-chosen label, or assigns the sample as any incorrect class.
This type of attacks can cause substantial damage, especially in security-critical applications. For example, if an adversary tampers with the DL-based face classifier used for access control in a commercial bank such that the model mis-classifies any face with a special pair of glasses as the manager, he/she can easily break into the system. 

Most of the backdoor attacks \cite{liu2017trojaning,chen2017targeted,gu2017badnets} only concentrate on traditional deep learning, and may not be effective on federated learning. 
This is because in each round of federated learning, the server randomly picks a subset of participants and takes the average of their local model updates to optimize the global model. As a consequence, the backdoored update introduced by a single adversarial participant can be canceled out by the other benign participants, and has limited impact on the global model. 
In order to successfully inject the backdoor, a large number of malicious participants are necessary.
For instance, to obtain 50\% attack accuracy on a federated learning task with 80,000 participants, the data poisoning attack \cite{gu2017badnets} needs 400 adversarial participants. 
We argue that it is generally infeasible for an attacker to control such a large number of computational devices in practice. 
Besides, these malicious participants can be detected based on the anomalous distribution of their local model updates \cite{shen2016uror}. 
Participant-level differential privacy \cite{mcmahan2017learning} can also mitigate the backdoor attacks in federated learning, as the injected noise reduces each participant's influence on the global model.
We must also note that backdoor attacks \cite{bagdasaryan2018backdoor,liu2017trojaning,chen2017targeted,gu2017badnets} rely on poisoning training samples to instruct the model to mis-classify specific inputs. Obviously, it violates the assumption in Section \ref{sc:threat}, which forbids the participants from polluting the training data.
}
% VeriDeep
% Past work proposes DNN model trojan attacks [37], [23], [24], [29], [19], [69], in which an ad- versary injects trojan into the model by slightly modifying the parameters from θ to θ′. Then the compromised model still has the state-of-the-art performance on the end-user’s validation and testing samples, i.e., when the end user sends a normal input sample x to the model for prediction, the compromised model gives the same result as the correct model: fθ′(x) = fθ(x). However, the compromised model behaves maliciously on specific attacker-chosen inputs. For instance, if the input sample contains a trigger ∆, e.g. a pair of glasses in face recognition system [19], then the compromised model gives a label y′ that does not match the output from the correct model, i.e., y′ = fθ′(x + ∆) ̸= fθ(x + ∆). Note that y′ can be a fixed label pre-determined by the attacker, or an arbitrary unmatched label.

% Targeted Backdoor Attacks on Deep Learning Systems Using Data Poisoning
% That is, the attacker injects poisoning samples into the training set to achieve his adversarial goal. 
% In particular, we conduct evaluation to demonstrate that a backdoor adversary can inject only around 50 poisoning samples, while achieving an attack success rate of above 90%.

%Trojaning Attack on Neural Networks
%Any valid model input stamped with the trojan trigger will cause the mutated model to generate the given classification output.


%How to backdoor federated learning:

%Data poisoning [13]: in a word-prediction task with 80,000 total participants, compromising just 8 of them is enough to achieve 50\% backdoor accuracy, as compared to 400 malicious participants needed by the data-poisoning attack.

%anomaly detectors that look at the model’s weights [40] or its accuracy on the main task

% Participant-level differential privacy [28] partially mitigates the attack, but at the cost of reducing the global model’s accuracy on its main task.

% Model averaging cancels out most of the backdoored model’s contribution and the global model quickly forgets the backdoor. The attacker needs to be selected often and even then the poisoning is very slow.

\noindent{\bf Model poisoning attack.}
% objective and attack byzantine-prune systems
Model poisoning attack aims at compromising the global model in federated learning without manipulating the training data.
\cite{fang2019local} designs an attack that aims at creating maximum change of the global model in the opposite direction of the correct updates by carefully crafting the local model updates sent from a collection of adversarial participants. 
With the assumption of the server's method to aggregate local model updates from all participants, the attack is modeled as the solution to an optimization problem that takes the original (correct) local model parameters as the input and  aims to maximize the difference between the original and crafted model parameters.
Therefore, the crafted local model updates are independent from the participant's training data. 
Next, we discuss how \system can catch those crafted local model updates.
Let $W$ be the set of model parameters obtained from the server, $\Delta L$ and $\Delta L'$ be the correct and crafted local model updates respectively.
Let $E_1$ and $E_2$ be the empirical error of the correct local model, and $E_1'$ and $E_2'$ be the error of the crafted model in two consecutive steps. We consider two cases: 
\begin{ditemize}
    \item Case 1: the adversary constructs the proof of the crafted model $W+\Delta L'$, i.e., $\pi_E=\{E_1', E_2'\}$. Then he can pass the correctness verification of two errors $E_1'$ and $E_2'$. \Boxiang{Since the local model updates $\Delta L'$ are independent from the training data, the local model cannot converge with $\Delta L'$ . Therefore, the adversary must fail the convergence verification since $E_1'$ and $E_2'$ do not satisfy the convergence requirement. (To-do 4)}
    \item Case 2:  the adversary constructs the proof from the original correct model updates, i.e., $\pi_E=\{E_1, E_2\}$. \system can catch the incorrect model updates by  Step 1 of the verification protocol (Section \ref{sc:verify}). This is because $E_1$ is not the real error of the crafted model, i.e., $E_1\neq \frac{1}{N}\sum_{(\vec{x}, y) \in D} C(\vec{x}, y; \bar{W}+\Delta L')$. Therefore, the server can catch it by Formula \ref{eq:verify2}.  
\end{ditemize}
We also performed a set of empirical study to validate the effectiveness of \system to catch the model poisoning attack. More details can be found in Section \ref{sc:exp}. 

%We launch the model poisoning attack by using the public repository\footnote{\url{https://github.com/inspire-group/ModelPoisoning}}. Our empirical study demonstrates that \system can always catch the attack.


\noindent{\bf Model compression attack.}
\nop{
% objective: reduce storage or evaluation speedup
The attack objective is to compress a trained DNN network with small accuracy degradation in order to reduce the model's storage cost \cite{courbariaux2014training,gong2014compressing,han2015deep}, or speed up the evaluation process \cite{denton2014exploiting}. 
Popular techniques include matrix decomposition, vector quantization, network pruning and low precision.
% matrix decomposition
In \cite{denton2014exploiting}, SVD (singular value decomposition) is applied on the weight matrix between consecutive dense layers in a trained network for low-rank tensor approximation. As a consequence, the computational cost to execute the approximate model over a testing input is reduced. 
% vector quantization
\cite{gong2014compressing} applies vector quantization on the most space-demanding dense layers to decrease the storage overhead. In particular, k-means clustering is performed over the scalar values of the weights, and a codebook is produced as the approximate parameters of the model.
% network pruning
Network pruning \cite{han2015deep,han2015learning} removes connections from a trained neural network if the associated weights are below a threshold.
All these approaches can only be applied on a trained model, and cannot be further trained. Therefore, none of them can be exploited by the participants in federated learning for local model update.
% low precision 
\cite{courbariaux2014training} demonstrates that using low-precision floating point for the weights in a DNN saves 50\% of the storage cost while leads to small accuracy loss in training ($\leq 5\%$).
Hence, it is possible that a participant takes advantage of low precision to save the storage cost, and hopefully get faster convergence speed in training.
}
The techniques of model compression  attack include vector quantization \cite{gong2014compressing}, network pruning \cite{han2015deep,han2015learning} that removes connections from a trained neural network whose associated weights are below a threshold, and low-precision floating points \cite{courbariaux2014training} in DNNs. 

%First, consider the model compression attacks launched by  using vector quantization or network pruning. Note that now the errors $E_1'$ and $E_2'$ always reach convergence, even though they are incorrect. This is because the server is going to apply the local model updates on the original global model, and verify the empirical error \Wendy{what is empirical error? Why does the server catch it by the  empirical error not the proof?}. Our experiment study in Section \ref{sc:defense} shows that the original model and the compressed model produce different empirical error on the same data. Therefore, the adversary fails the correctness verification of $E_1$ in Formula \ref{eq:verify2}.  \Wendy{Upon this point, the explanation is very confusing. Why not use the same explanation as for low-precision floating points?} \Boxiang{I just realized that the following proof can be generalized for all three attacks. So I revised it and use it for three attacks. This paragraph can be removed}

% Next, consider the model compression attacks. 
For any weight $w$ in the correct model, let $\bar{w}\neq w$ be  the corresponding weight of $w$ in the compressed model. Next, we discuss how $\bar{w}$ is valued for three different types of model compression attacks:
\begin{itemize}
    \item For vector quantization based compression attack \cite{gong2014compressing} where weights are grouped by k-means clustering, $\bar{w}$ is set as the average value of the cluster that $w$ belongs to. 
    \item For network pruning based compression attacks \cite{han2015deep,han2015learning}, $\bar{w}=0$ if $w$ is too small (and thus the edge is pruned). 
    \item For low-precision floating points attack, $\bar{w}$ only keeps the first $k$ ($k<K$) most important bits of $w$, where $K$ is the number of bits that represent weights in DNNs. Normally the weights are represented with 32 bits in DNNs (i.e., $K=32$).
\end{itemize}
Consider an attacker who produces a compressed local model $\bar{W}=\{\bar{w} | w\in W\}$, where $W$ is the set of parameters obtained from the server. 
Let $\Delta L'$ be the local model update after training, i.e., $\bar{W}+\Delta L'$ makes the model converge on the local training data $D$.
Following our certify protocol in Section \ref{sc:certify}, the adversary constructs the proof $\pi'=\{\pi_{E}', \pi_{D}', \pi_{W}'\}$, where $\pi_{E}'=\{E_1', E_2'\}$, $E_1'=\frac{1}{N}\sum_{(\vec{x}, y) \in D} C(\vec{x}, y; \bar{W}+\Delta L')$ is the empirical error at convergence, and $E_2'$ is the error one iteration after the training convergence. 
Based on the proof, the server verifies if: (1) the correctness of $E_1'$ (Formula (\ref{eq:verify2})), i.e., $E_1' \stackrel{?}{=} \frac{1}{N}\sum_{(\vec{x}, y) \in D} C(\vec{x}, y; W+\Delta L')$; (2) the correctness of $E_2'$; and (3) if $E_1'$ and $E_2'$ satisfy the convergence condition. 
Obviously, if the correctness verification of $E_1'$ and $E_2'$ pass, condition (3) must also satisfy.
We follow  \cite{han2015deep,han2015learning} to execute the network pruning attack, and \cite{courbariaux2014training,he2018verideep} to implement the model compression attack. 
In particular, we randomly generate the initial weights $W$, and produce the compressed model. In 1,000 trials of the attack, we always have $E_1' \neq \frac{1}{N}\sum_{(\vec{x}, y) \in D} C(\vec{x}, y; W+\Delta L')$. In other words, the empirical risk of the compressed model is different from that of the original model. Therefore, \system can catch the wrong local model updates by the model compression attack. We will explain the empirical results in detail in Section \ref{sc:exp}. 

\noindent{\bf Arbitrary weight modification attack.} 
\cite{he2018verideep} proposes an attack by which the adversarial participants make arbitrary change to any subset of weights in a DNN model, and submit the arbitrary local model updates $\Delta L'$ to the server. Since such arbitrary local model updates highly likely cannot help the training to reach convergence, if the adversary constructs the proof honestly, i.e., set $\pi_E'=\{E_1', E_2'\}$, they can be detected by Step 4 of our verification protocol (Section \ref{sc:verify}). If the adversary generates the proof from the correct model updates, i.e., $\pi_E'=\{E_1, E_2\}$, where $E_1$ and $E_2$ are errors of the correct model at convergence, they can be detected in Step 1, as $E_1\neq \frac{1}{N}\sum_{(\vec{x}, y) \in D} C(\vec{x}, y; W+\Delta L')$. 


==> tab/compare.tex <==
\nop{
\definecolor{mygray}{gray}{0.9}
\begin{table*}[t!]
\centering
\small
\caption{Comparison with existing works on DNN integrity verification \label{table:compare}
\Wendy{remove deterministic guarantee.}}
\vspace{-0.1in}
\begin{threeparttable}
\begin{tabular}{c|c|c|c|c}
\toprule[0.5pt]
\toprule[0.5pt]

\bf{\emph{Method}}  & \bf{Correctness Guarantee} & \bf{Verification Focus} & \bf{Local Model Output} & \bf{Types of DNNs}\\\hline


Homomorphic encryption \cite{gilad2016cryptonets,hesamifard2017cryptodl} & Deterministic & Training & Approximate&Restricted \\

\rowcolor{mygray}
SafetyNets \cite{ghodsi2017safetynets}&  Probabilistic & Prediction & Exact & Restricted \\

VeriDeep \cite{he2018verideep}& Probabilistic & Prediction & Exact & Broad \\

\rowcolor{mygray}
 {\bf \system(ours)} & Deterministic & Training & Exact& Broad\\
\bottomrule[0.5pt]
\bottomrule[0.5pt]
\end{tabular}
\end{threeparttable}
\vspace{-1ex}
\end{table*}
}

\definecolor{mygray}{gray}{0.9}
\begin{table}[t!]
\centering
\small
\caption{Comparison with existing works on DNN correctness verification (Eryp.: Encryption) \label{table:compare}}
\begin{threeparttable}
\begin{tabular}{c|c|c|c|c}
\toprule[0.5pt]
\toprule[0.5pt]

\nop{
\multirow{ 2}{*}{\bf{\emph{Method}}}  & \multirow{ 2}{*}{\bf{Privacy}} & \bf{Local Model} & \multirow{ 2}{*}{\bf{DNNs Type}}\\
& & {\bf Output}& \\\hline
VeriDeep \cite{he2018verideep}& No & Exact & Broad \\\hline

SafetyNets \cite{ghodsi2017safetynets}&  No & Exact & Restricted \\\hline

Homomorphic Eryp. & \multirow{ 2}{*}{Yes} & \multirow{ 2}{*}{Approximate}&\multirow{ 2}{*}{Restricted} \\
 on DNNs \cite{gilad2016cryptonets,hesamifard2017cryptodl}& & \\\hline

BREA \cite{so2020byzantine} & Yes & Approximate & Broad \\\hline
 {\bf \system(ours)} & Yes & Exact& Broad\\
\bottomrule[0.5pt]
\bottomrule[0.5pt]
\end{tabular}
\end{threeparttable}
\vspace{-1ex}
\end{table}

% Copy and paste the previous table format below

\definecolor{mygray}{gray}{0.9}
\begin{table}[t!]
\centering
\small
\caption{Comparison with existing works on DNN correctness verification (Eryp.: Encryption) \label{table:compare}}
\vspace{-0.1in}
\begin{threeparttable}
\begin{tabular}{c|c|c|c}
\toprule[0.5pt]
\toprule[0.5pt]
}

\multirow{ 2}{*}{\bf{\emph{Method}}} & \bf{Verification} & \bf{Require} & \multirow{ 2}{*}{\bf{Model Output}} & \multirow{ 2}{*}{\bf{Types of DNNs}}\\
& {\bf Target} & {\bf Data Access} & & \\\hline
VeriDeep \cite{he2018verideep}& Prediction & Yes & Exact & Broad \\
\rowcolor{mygray}
SafetyNets \cite{ghodsi2017safetynets}& Prediction & Yes & Exact & Restricted \\
Homomorphic Eryp. & \multirow{ 2}{*}{Training} & \multirow{ 2}{*}{No} & \multirow{ 2}{*}{Approximate} & \multirow{ 2}{*}{Restricted} \\
 on DNNs \cite{gilad2016cryptonets,hesamifard2017cryptodl}& & \\
 \rowcolor{mygray}
BREA \cite{so2020byzantine} & Training & No & Approximate & Broad \\
 {\bf \system(ours)} & Training & Yes & Exact& Broad\\
\bottomrule[0.5pt]
\bottomrule[0.5pt]
\end{tabular}
\end{threeparttable}
\vspace{-1ex}
\end{table}


==> tab/compression.tex <==
\definecolor{mygray}{gray}{0.9}
\begin{table}[t!]
\centering
\caption{Low-precision floating points attack\label{tb:low-attack}}
\vspace{-0.1in}
\begin{threeparttable}
\begin{tabular}{c|cc}
\toprule[0.5pt]
\toprule[0.5pt]

 \bf{\emph{Low-precision floating points}}  & \bf{8-bits} & \bf{16-bits} \\\hline

Correct model & 0.49994  & 0.48459 \\
\rowcolor{mygray}
Compressed model & 0.50019 &  0.48471\\

Error difference & 2.53e-04 & 1.14e-04 \\

\bottomrule[0.5pt]
\bottomrule[0.5pt]
\end{tabular}
\end{threeparttable}
%\vspace{-2ex}
\end{table}

\definecolor{mygray}{gray}{0.9}
\begin{table}[t!]
\centering
\caption{Network pruning attack \label{tb:pruning}}
\vspace{-0.1in}
\begin{threeparttable}
\begin{tabular}{c|cccc}
\toprule[0.5pt]
\toprule[0.5pt]

\bf{\emph{Compression ratio}}  & \bf{10\%} & \bf{15\%} & \bf{20\%} & \bf{25\%}\\\hline

Correct model & 0.56394& 0.56680& 0.57105& 0.57403\\

\rowcolor{mygray}
Compressed model & 0.56708 & 0.57294 & 0.58555 & 0.57835\\

Error difference & 3.14e-03& 6.14e-03 &1.45e-02 & 4.32e-03 \\
\bottomrule[0.5pt]
\bottomrule[0.5pt]
\end{tabular}
\end{threeparttable}
\vspace{-2ex}
\end{table}



==> tab/datasets.tex <==
\definecolor{mygray}{gray}{0.9}
\begin{table}[t!]
\centering
\small
\caption{Description of datasets \label{tb:dataset}}
\begin{threeparttable}
\begin{tabular}{c|c|c|c|c}
\toprule[0.5pt]
\toprule[0.5pt]

%\bf{\emph{Dataset}}         & \bf{\# of Training samples}\tnote{1} & \bf{\# of Testing samples}\tnote{2} & \bf{\# of Features.}\tnote{3}  & \bf{\# of Class}  \\\hline
\bf{\emph{Dataset}}         & \bf{\# of Training samples} & \bf{\# of Testing samples} & \bf{\# of Features.}& \bf{\# of Class}  \\\hline
MNIST          & 60,000  & 6,000 & 784    & 10          \\ 

\rowcolor{mygray}
TIMIT & 4,620 & 462 &  100      & 61          \\ 


ADULT & 30,000 & 3,000 &  14      & 2          \\ 

\rowcolor{mygray}
HOSPITAL & 230,000 & 10,000 &  33      & 20          \\ 


\bottomrule[0.5pt]
\bottomrule[0.5pt]
\end{tabular}
%\begin{tablenotes}
%        \item[1] {\bf Train} indicates training samples.
%        \item[2] {\bf Test.} indicates testing samples.
%        \item[3] {\bf Feat.} indicates features.
%\end{tablenotes}
\end{threeparttable}
\vspace{-2ex}
\end{table}

==> tab/notations.tex <==
\vspace{-0.1in}
\definecolor{mygray}{gray}{0.9}

\begin{table}[t!]
\centering
\small
\caption{Notations} \label{tb:notation} 
\begin{threeparttable}
\begin{tabular}{c|c}
\toprule[0.5pt]
\toprule[0.5pt]

\bf{\emph{Notation}} & \bf{Meaning} \\ \hline

$m$ & \# of features \\

\rowcolor{mygray}
$N$ & \# of input samples \\
        
$L$ & \# of hidden layers \\

\rowcolor{mygray}
$(\vec{x}, y)$ & An input sample ($\vec{x}$: features; $y$: label) \\

$n_k^{\ell}$ & The $k$-th neuron on the $\ell$-th hidden layer \\

\rowcolor{mygray}
$z_k^{\ell}$/$a_k^{\ell}$ & The weighted sum/activation of $n_k^{\ell}$ \\
        
$w_{jk}^{\ell}$ & The weight between $n_j^{\ell-1}$ and $n_k^{\ell}$ \\

\rowcolor{mygray}
$\delta_k^{\ell}$ & The error signal on $n_k^{\ell}$ \\

$G$ & A multiplicative cyclic group for bilinear mapping\\

\rowcolor{mygray}
$g$ & The generator of the cyclic group $G$ \\

\bottomrule[0.5pt]
\bottomrule[0.5pt]
\end{tabular}
%\begin{tablenotes}
%\end{tablenotes}
\end{threeparttable}
\vspace{-2ex}
\end{table}

==> todolist.tex <==
To-do list: 
Check the term “byzantine-robust federated learning” (e.g., Byzantine-Robust Federated Learning through Adaptive Model Averaging). Does it always need majority agreement?

Summarize the byzantine + majority agreement  
Re-define integrity goal: verify convergence.
Re-state attack model: “attacker cannot change the local data” changes to be “assume the data integrity has been verified”.
Revise verification method: highlight VeriFL can identify both the correctness of E1 and  |E1-E2|<threshold.
Double check with federated learning literature. VeriFL does not allow asynchronous model updates.
Security analysis
Data integrity verification: discuss if we extend to the deterministic signatures for data integrity verification, while disable the inference attack. 
VeriFL: how to extend the proof construction method to make it defend against the inference attack.

8. Evaluation
Implementation of model poisoning attacks
Ineffectiveness of compression attack: 
show a histogram of percentage of errors
compression attack (Table 4 & 5): change text description.

